Designing Fair Ranking Schemes

Items from a database are often ranked based on a combination of multiple criteria. A user may have the flexibility to accept combinations that weigh these criteria differently, within limits. On the other hand, this choice of weights can greatly affect the fairness of the produced ranking. In this paper, we develop a system that helps users choose criterion weights that lead to greater fairness. We consider ranking functions that compute the score of each item as a weighted sum of (numeric) attribute values, and then sort items on their score. Each ranking function can be expressed as a vector of weights, or as a point in a multi-dimensional space. For a broad range of fairness criteria, we show how to efficiently identify regions in this space that satisfy these criteria. Using this identification method, our system is able to tell users whether their proposed ranking function satisfies the desired fairness criteria and, if it does not, to suggest the smallest modification that does. We develop user-controllable approximation that and indexing techniques that are applied during preprocessing, and support sub-second response times during the online phase. Our extensive experiments on real datasets demonstrate that our methods are able to find solutions that satisfy fairness criteria effectively and efficiently.

==> discussions.tex <==
\subsection{Discussion}\label{sec:discussions}

\stitle{Designing Diverse Ranking Schemes.}
Diversification of the query results has always been an important data retrieval topic~\cite{diversity, boyce1982beyond, agrawal2009diversifying}. Different definitions of diversity include similarity function based~\cite{chen2006less} and topic based~\cite{agrawal2009diversifying} definitions. A nice property of the techniques proposed in this paper is that those are independent on the choice of fairness function, and in fact, one can replace the fairness oracle with any binary-output function that takes an ordering of the items as the input. This makes this paper suitable for a general range of diversity definitions as well. All is needed is to pass the orderings to the diversity oracle (instead of a fairness oracle), and all the claims in the paper remain valid.

%\stitle{Further optimizations based on the fairness model details.}
\subsection{Optimizations based on the fairness model}
\label{sec:opt:fairness}

In this paper, we designed techniques for a general fairness definition that takes an ordering of the items as the input and decides whether it meets the fairness requirements. However, additional information about the fairness model can help optimize the techniques. For example, knowing that $\mathcal{O}$ investigates fairness only within the top-$k$ of the ordering~\cite{DBLP:conf/cikm/ZehlikeB0HMB17} can help in ignoring the items that do not belong to the $k^{th}$ convex layer~\cite{chang2000onion}, as those will never appear within the top-$k$. This reduces the complexity of the arrangement from $n^{2(d-1)}$ to $n_k^{2(d-1)}$, where $n_k$ is the number of items in the top $k$ convex layers.

\stitle{Scaling up preprocessing for large datasets.}\label{subsec: sampling.}
\subsection{Sampling-based approximation}
\label{sec:opt:sample}
We finally discuss a sampling strategy for the large datasets, that guarantees finding ``close to satisfactory'' results.
A critical requirement of our system is to be efficient in the online processing of the user queries, and it is fine for it to spend more time in the offline preprocessing.
As discussed in \S~\ref{sec:md} and \S~\ref{sec:speedup}, the proposed offline algorithms in this paper are polynomial for a fixed value of $d$.
In addition, using the arrangement tree (c.f. \S~\ref{sec:md}), as well as the techniques proposed in \S~\ref{sec:speedup}, helps in speeding up the process in practice.
However, due to the curse of dimensionality, preprocessing can still be slow, particularly for a large number of items.  For these situations, we propose a sampling-based preprocessing strategy.

The main idea is that a uniform sample of the data maintains the underlying properties of the data distribution. Therefore, if a function is satisfactory for a dataset, it is {\em expected} to be satisfactory for a uniformly sampled subset.  \julia{What follows in this paragraph is defensive, I suggest removing, and replacing with a preview of the relevant experimental results instead.  I'll take care of this but let me know if you object.} As a result, if one does the preprocessing on a uniformly sampled subset, rather than returning a function $f'$ that is satisfactory, when answering the users' queries, it returns a function $f'$ that is {\em expected} to be satisfactory. That is, the deviation of its ordering from a a satisfactory ordering, with a high confidence, is very low. Of course, providing the precise statements depends on the choice of ranking model.
Also, the proposed techniques in this paper are provided for a fixed number of dimensions. For the variable high dimensional situations, the problem is NP-complete, following the complexity of the arrangement. We consider extending the application for the variable number of dimensions for the future work.

%\stitle{The effect of bias in the individual scalar attributes.}



==> geo.tex <==
\section{Some geometric concepts}\label{subsec: georeview}
\textcolor{blue}{TBD!}
The basic data structure in $\mathbb{R}^d$ is a point, which is known as the zero dimensional structure.
In the euclidean space, a line is a one dimensional 
Line is the one dimensional data structure that pass
A line passes Between every pair of points
hyperplane, hyperplane representation, intersection of hyperplanes, 
show that the equation of each hyperplane in the form of $\sum\limits_{j=1}^d A_j x_j = D$ can be rewritten as $\sum\limits_{j=1}^d \frac{A_j}{D}x_j = 1$, if $D\neq 0$.

-----------------------

Without loss of generality, considering the general positioning assumption, for the ease of explanation, we assume that no two items have the rank equality passing through the angle $\langle 0,\cdot, 0 \rangle$.
Thus, any hyperplane can be presented in the form of\footnote{\small The hyperplanes passing through the point $\langle 0,\cdots, 0 \rangle$, we simply consider $\sum\limits_{k=1}^d A_k x_k  = 0$.}:
\begin{align}\label{eq:hp}
\sum\limits_{k=1}^d A_k x_k = 1
\end{align}
--------------------------

----------- arrangement ----------

----------- polar v.s. scalar coordinate system. how to compute the polar and scalar of a point in $\mathbb{R}^d$ -------------\\
do not forget to mention the way that angles are considered $\rightarrow$ each angle $\theta_i$ is computed against the plane $x_i=0$. 
